End-to-End Ascent-Entry Mission Performance Optimization Using Gaussian Quadrature Collocation

The performance optimization for a combined ascent-entry mission subject to constraints on heating rate and heating load is studied. The ascent vehicle is modeled as a three-stage rocket that places the vehicle onto a suborbital exo-atmopheric trajectory after which the vehicle undergoes an unpowered entry and descent to a vertically downward terminal condition. The entry vehicle is modeled as a high lift-to-drag ratio vehicle that is capable of withstanding high levels of thermal and structural loads. A performance index is designed to improve control margin while attenuating phugoid oscillations during atmospheric entry. Furthermore, a mission corresponding to a prototype launch and target point is used in this study. The trajectory optimization problem is formulated as a multiple-phase optimal control problem, and the optimal control problem is solved using an adaptive Gaussian quadrature collocation method. A key aspect of the optimized trajectories is that, for particular ranges of maximum allowable heating rate and heating load during entry, relatively small adjustments made during ascent can potentially decrease the control effort required during atmospheric entry. Outside of these ranges for maximum allowable heating rate and heating load, however, it is found that the required control effort increases and eventually saturates the commanded angle of attack upon initial descent. The key features of the optimized trajectories and controls are identified, and the approach developed in this paper provides a systematic method for end-to-end ascent-entry trajectory optimization.

==> temp.tex <==
BGphases.eps
MinIVCLlow.eps
MinIVCDlow.eps
MinIVLDlow.eps
MinIVCLhigh.eps
MinIVCDhigh.eps
MinIVLDhigh.eps
CAVCL.eps
CAVCD.eps
CAVLD.eps
CAVModelData.eps
sigK.eps
sigKfpa.eps
sigKfpa_enlarged.eps
sigKh.eps
sigKv.eps
sigKQdot.eps
sigKn.eps
sigKaoa.eps
sigKbank.eps
HRcost.eps
HRaoa.eps
HRh.eps
HRv.eps
HRQdot.eps
Qcost.eps
Qaoa.eps
Qh.eps
Qv.eps
FailurePoints.eps
CombinedQdot.eps
CombinedGload.eps
Combinedaoa.eps
Combinedh.eps
Combinedv.eps


==> temp2.tex <==
sigKq.eps

